DDPEN: Trajectory Optimisation With Sub Goal Generation Model

Differential dynamic programming (DDP) is a widely used and powerful trajectory optimization technique, however, due to its internal structure, it is not exempt from local minima. In this paper, we present Differential Dynamic Programming with Escape Network (DDPEN) - a novel approach to avoid DDP local minima by utilising an additional term used in the optimization criteria pointing towards the direction where robot should move in order to escape local minima. In order to produce the aforementioned directions, we propose to utilize a deep model that takes as an input the map of the environment in the form of a costmap together with the desired goal position. The Model produces possible future directions that will lead to the goal, avoiding local minima which is possible to run in real time conditions. The model is trained on a synthetic dataset and overall the system is evaluated at the Gazebo simulator. In this work we show that our proposed method allows avoiding local minima of trajectory optimization algorithm and successfully execute a trajectory 278 m long with various convex and nonconvex obstacles.

==> chapters/2_related.tex <==
\section{Related Work}
% Motion prediction has become a separate task primarily motivated by the effective navigation of the mobile robot in the social environment. 
% Early works were aimed at describing the model of human movement by model-based approach \cite{sfm,hsfm}. 
% In some cases of a short prediction horizon or movement on a limited straight sidewalk, the simple linear interpolation or Constant Velocity Model (CVM)\cite{cvm} can show fairly good accuracy. Still, when there are a lot of pedestrians, it is also necessary to take into account their interaction between each other.
% This type of interaction can be modeled by Social Force Model (SFM)\cite{sfm} or more related to the human movement model the Headed Social Force Model (HSFM)\cite{hsfm}, which directly take into account such interactions in their model of motion.
% However, the accuracy of these models strongly depends on how well the destination point is selected, which is used as input data. 

% In the last years, deep learning approaches have become dominant in the task of Human motion prediction.
% Modern deep learning frameworks allow optimizing algorithm computation time by utilizing GPU resources. For example, it has been shown \cite{mpdm, sigma-nn} how empirical models can be packed into layers-like neural network structures that can use optimized gradient descent to calculate backpropagation loss efficiently.
% \par
%1 Social LSTM
% One of the most popular works that use deep learning approach is Social-LSTM\cite{social-lstm} show a simple but effective way of using Recurrent Neural Networks (RNN)\cite{rnn} variant named Long Short Term Memory (LSTM)\cite{lstm} blocks for learning general human movement and predict their future trajectories.
% \par
%1.1 SoPhie
% There are another deep learning approach based on Generative Adversarial Network(GAN) named SoPhie\cite{sophie}, which leverages path history information with scene context information, using images. 
\par
%2 Trajectron++
% Another deep learning approach utilizes a graph-structured data model. 
% Trajectron \cite{trajectron} and its second version Trajectron++ \cite{trajectronplusplus}  - multi-agent behavior prediction model that accounts for the dynamics of the agents, produces predictions possibly conditioned on potential future robot trajectories which can effectively use heterogeneous data about the surrounding environment.
\par
% PecNet \cite{pecnet} propose estimation of a latent belief distribution modeling the pedestrians’ possible endpoints, which are used to predict trajectories. 
% This approach has shown good prediction accuracy, and also it provides additional information about possible trajectories in the outputs, which can be taken into account in trajectory planning step.
% The Perceiver \cite{perceiver} propose novel general perception architectures with latent transformers similar to GPT-2 architecture\cite{gpt2,transformer}, and cross-attention blocks. 
% This work is from a different field of image processing, but despite this, we used some of the ideas from this approach, which we adapted for a human motion prediction field.
% The main advantage of such an approach is a simplicity and flexibility of architecture while performing on par with the current state of the art\cite{trajectron, trajectronplusplus, sophie}.

